Optimal Control of Dynamic Bipartite Matching Models

A dynamic bipartite matching model is given by a bipartite matching graph which determines the possible matchings between the various types of supply and demand items. Both supply and demand items arrive to the system according to a stochastic process. Matched pairs leave the system and the others wait in the queues, which induces a holding cost. We model this problem as a Markov Decision Process and study the discounted cost and the average cost problem. We fully characterize the optimal matching policy for complete matching graphs and for the N -shaped matching graph. In the former case, the optimal policy consists of matching everything and, in the latter case, it prioritizes the matchings in the extreme edges and is of threshold type for the diagonal edge. In addition, for the average cost problem, we compute the optimal threshold value. For more general graphs, we need to consider some assumptions on the cost of the nodes. For complete graphs minus one edge, we provide conditions on the cost of the nodes such that the optimal policy of the N-shaped matching graph extends to this case. For acyclic graphs, we show that, when the cost of the extreme edges is large, the optimal matching policy prioritizes the matchings in the extreme edges. We also study the W-shaped matching graph and, using simulations, we show that there are cases where it is not optimal to prioritize to matchings in the extreme edges.

==> Heuristic.tex <==


\section{General Bipartite Graphs}

\begin{figure}[b]

\centering
\includegraphics[scale=0.48]{Simulations/AsymptoticArrival_HighCostWorkload_2.png}
\caption{NN model. Average cost of our heuristic (with a threshold of $0$ in $d_1$, $9$ in $s_3$ and $0$ in $d_2$ and $s_2$), max-weight policy and hMWT the heavy-traffic optimal policy established in \citep{BoundedRegret} (with parameters $D=\{d_3\}$, $\beta=2$, $\kappa=10$, $\theta=1$, $\delta^+ =0.01$ and $\bar{n}_u=8$).}
\label{fig:NNexample1}
\end{figure}

\begin{figure}[h]

\centering
\includegraphics[scale=0.48]{Simulations/NormalArrival_HighCostWorkload_2.png}
\caption{NN model. Average cost of our heuristic (with a threshold of $0$ in $d_1$, $1$ in $s_3$ and $0$ in $d_2$ and $s_2$), max-weight policy and hMWT the heavy-traffic optimal policy established in \citep{BoundedRegret} (with parameters $D=\{d_3\}$, $\beta=2$, $\kappa=10$, $\theta=1$, $\delta^+ =0.01$ and $\bar{n}_u=8$).}
\label{fig:NNexample2}
\end{figure}

%

In this section, we investigate the optimal matching policy for general bipartite graphs. The natural extension of the optimal matching policy identified in the case N would be to prioritize the end edges. However, the concept of end edges only make sense for acyclic graphs. Therefore, we  present first a heuristic for the case of acyclic bipartite graphs, that is an extension of the threshold type policy for the $N$-case (see Definition~\ref{def:threshold_policy}). 

Our heuristic gives priority to the end edges and puts thresholds on vertices that are incident to those end edges. Then, the policy gives priority to the edges that are adjacent to the end edges and puts thresholds on vertices that are incident to those edges. We repeat this process until all edges are exhausted. This means that our heuristic first matches everything in the end edges. Then it matches everything in the adjacent edges that is above the thresholds (set on the incident vertices), and so on.
For general graphs, our heuristics uses the max-weight policy for the cycles and the heuristic for the acyclic graphs for the remaining of the graph. Priority is given to the nodes that are not a part of a cycle.  Ties between two acyclic branches can be broken using the max-weight policy. 

We consider the NN model, which is formed by three supply nodes and three  demand nodes (see Figure~\ref{fig:NN}). In this model, the end edges are $(d_1,s_1)$ and $(d_3, s_3)$. Thus, our heuristic first matches all $(d_1,s_1)$ and all $(d_3, s_3)$. Then, it matches every $(d_1,s_2)$ above the threshold in $d_1$ and every $(d_2,s_3)$ above the threshold in $s_3$. Finally, it matches every $(d_2,s_2)$ above the threshold in $d_2$ and $s_2$. 
We compare the average cost of our heuristic with various policies in two different settings. We consider the max-weight policy which is well known in the literature and performs well in many applications. The decision rule for the max-weight policy is given as the solution of the following optimization problem:
\[
u_{MW} = \text{argmax} \{u\cdot \nabla h(x): u\in U_x \},\; x\in\mathcal{X},
\]
where $h(x)=\sum_{i\in \mathcal{D}\cup\mathcal{S}} c_i x_i^2$. We also consider the hMWT policy which was proved asymptotically optimal in heavy-traffic regime in \cite{BoundedRegret}.

For our fist example, we want to compare our heuristic with results from \cite{BoundedRegret} and thus, we choose the same arrival rates and costs. This means that $\alpha_1=\frac36$, $\alpha_2=\frac26$, $\alpha_3=\frac16$, $\beta_1=\frac26 -\frac{\delta}{2}$, $\beta_2=\frac36 -\frac{\delta}{2}$ and $\beta_3=\frac16 +\delta$ (with $\delta=0.06$) and $c_{d_1}=c_{s_1}=1$, $c_{d_2}=c_{s_2}=2$ and $c_{d_3}=c_{s_3}=3$. In Figure~\ref{fig:NNexample1}, we show the result of the numerical experiments we have performed for this model. As it can be observed, our heuristic performs better than max-weight and is not far from hMWT.

We tested our heuristic in a second example which is not close to a heavy-traffic regime. For the arrival rates, we choose similar rates as in the first example but with $\delta=0.5$ and for the costs, we choose the same as in the first example. In Figure~\ref{fig:NNexample2}, we show that our heuristic outperforms the other policies.

The Python code for both examples can be found at \cite{Code}.



